CCStereo: Audio-Visual Contextual and Contrastive Learning for Binaural Audio Generation

Binaural audio generation (BAG) aims to convert monaural audio to stereo audio using visual prompts, requiring a deep understanding of spatial and semantic information. However, current models risk overfitting to room environments and lose fine-grained spatial details. In this paper, we propose a new audio-visual binaural generation model incorporating an audio-visual conditional normalisation layer that dynamically aligns the mean and variance of the target difference audio features using visual context, along with a new contrastive learning method to enhance spatial sensitivity by mining negative samples from shuffled visual features. We also introduce a cost-efficient way to utilise test-time augmentation in video data to enhance performance. Our approach achieves state-of-the-art generation accuracy on the FAIR-Play and MUSIC-Stereo benchmarks.

==> section/old_abstract.tex <==
Binaural audio generation (BAG) aims to convert monaural audio to stereo audio using visual prompts, requiring a deep understanding of spatial and semantic information. 
% 
The success of the BAG systems depends on the effectiveness of cross-modal reasoning and spatial understanding. 
Current methods have explored the use of visual information as guidance for binaural audio generation. However, they rely solely on cross-attention mechanisms to guide the generation process and lack dense spatial understanding. This limitation increases the risk of overfitting to specific room environments and results in the loss of fine-grained spatial details, ultimately constraining model performance.
% 
In this paper, we address the aforementioned issues by introducing a new audio-visual binaural generation model incorporating an audio-visual conditional normalisation layer that dynamically aligns the mean and variance of the target difference audio features using visual context, along with a new contrastive learning method to enhance spatial sensitivity by mining negative samples from shuffled visual features.
We also introduce a cost-efficient way to utilise test-time augmentation in video data to enhance performance.
% 
Our approach achieves state-of-the-art generation accuracy on the FAIR-Play and MUSIC-Stereo benchmarks. 
\textcolor{urlblue}{Code will be released.} 

==> section/old_intro.tex <==

\section{Introduction}
\label{sec:intro}

% -- Introduce Binaural audio
% -- Introduce the current problem definition and potential problem.
% -- How the existing paper address these issues
% -- Then what is the problem with the existing method
% -- What we propose to address this issue


Binaural audio is gaining significant attention in streaming media, revolutionising how listeners experience sound in a digital environment. This technology finds applications in various domains, including virtual reality (VR) \cite{hoeg2017binaural}, 360-degree videos \cite{morgado2018self}, and music \cite{griesinger1990binaural}.
By simulating a two-dimensional soundscape, binaural audio creates a deeply immersive experience, allowing listeners to feel as if they are physically present within the auditory scene.

% -- Exisiting method 
% (1) Improve realisation of the spatial information / Enhancing the spatial reasoning
% Enhance positional information (Depth)
% Improve cross-model interaction (Multi-Attention Audio-Visual Fusion)
% Introduce proxy text (sep-stereo, multi-task learning, visually Liu.)
% Room Environment.
% (2) Overfitting issue (Visually Xu)

\begin{figure}
    \centering
    \includegraphics[width=.9\linewidth]{figures/icme2025-motivation.drawio.pdf}
    \vspace{-10pt}
    \caption{
    Comparison between previous mono-to-binaural methods~\cite{gao20192,zhou2020sep} (top) and our proposed CCStereo framework (bottom). While prior approaches primarily rely on implicit global alignment, CCStereo explicitly targets three key aspects of the spatialisation process: (1) \textbf{align} establishes audio-visual correspondence; (2) \textbf{adjust} the predicted stereo features by matching the mean and variance of the target; and (3) applying visual perturbations during inference to robustify to the prediction. In addition, CCStereo incorporates dense contrastive learning to improve spatial sensitivity through discriminative supervision across visual contexts.
    }
    \vspace{-10pt}
    \label{fig:motivation}
    \Description[Comparison between previous methods and our method.]{Comparison between previous methods and our method.}
\end{figure}

Binaural audio recording typically requires specialised hardware like dummy head systems~\cite{gao20192}. These systems are costly and lack portability, making them impractical for everyday use. To address this, researchers have developed methods to spatialise audio from monaural recordings, known as binaural audio generation (BAG)~\cite{gao20192,zhou2020sep,xu2021visually}. These methods use visual information to estimate the differential audio between left and right channels. However, existing frameworks often rely on simple feature fusion strategies, which may struggle to capture complex visual-spatial relationships, limiting their generalisability and performance.
% 
To better utilise the visual information, previous works~\cite{gao20192,zhou2020sep,xu2021visually,parida2022beyond,li2024cross,li2024cyclic} have explored various strategies to enhance semantic and spatial awareness across modalities. These approaches aim to improve cross-modal feature interaction~\cite{zhou2020sep,xu2021visually,parida2022beyond,zhang2021multi}, strengthen spatial understanding~\cite{garg2021geometry,li2024cross,li2024cyclic}, and incorporate 3D environmental cues~\cite{garg2021geometry}. 
%
% \hl{
Despite promising results, these methods still lack a dense spatial understanding, which limits their ability to accurately capture local spatial relationships between multimodal features.
% }


In addition, existing models remain prone to overfitting the training environment due to their reliance on specific data distributions and insufficient regularisation mechanisms. These issues often result in limited generalisation to diverse or unseen scenarios.
Unfortunately, the structure of the widely used FAIR-Play~\cite{gao20192} dataset fails to address this concern, as a significant amount of scene overlap has been observed between the training and testing sets~\cite{xu2021visually}, resulting in overly optimistic evaluation results on the current benchmark. 
Xu et al.~\cite{xu2021visually} tackled this issue by reorganising the dataset based on clustering results of scene similarity. 
Additionally, methods involving training on synthetic stereophonic data from external sources~\cite{zhou2020sep, xu2021visually} and incorporating depth estimation~\cite{parida2022beyond} have also shown potential in mitigating the overfitting problem.
% IP-Adaptor
However, these methods still rely on concatenation or cross-attention to guide the generation process. While cross-attention excels in blending features from different modalities (i.e., representation fusion~\cite{xu2013survey,li2018survey,baltruvsaitis2018multimodal,xu2021visually, xuan2020cross}), it is weak at aligning and maintaining spatial fidelity in the audio, making it less effective for integrating fine-grained conditioning information.


In this paper, we introduce a novel U-Net-based generation framework, named as \underline{C}ontextual and \underline{C}ontrastive \underline{Stereo}phonic Learning (CCStereo), which aims to address the aforementioned challenges.
% 
The framework consists of a visually adaptive stereophonic learning method that enhances cross-modal ``alignment'' and enables ``adjustment'' to the generation process based on the provided spatial information, along with a robustified and cost-effective inference strategy, as shown in Fig.~\ref{fig:motivation}.
% 
Unlike previous methods that rely solely on concatenated~\cite{gao20192,zhou2020sep,xu2021visually,li2024cross,liu2024visually} or cross-attended~\cite{zhang2021multi} features for differential audio generation, we adopted the concept of conditional normalisation layers~\cite{huang2017arbitrary,nam2018batch} from image synthesis field to control the generation process through estimated mean and variance shifts informed by visual context. 
% 
Additionally, we propose a novel audio-visual contrastive learning method that improves the model's spatial sensitivity by enforcing feature discrimination across the anchor frame, nearby frames, and the spatially shuffled anchor frame. This encourages the model to learn more discriminative representations of different object locations and their corresponding generated spatial audio, as illustrated by the simulated position change of the piano in Fig.~\ref{fig:motivation}.
% 
Moreover, the widely used sliding window inference strategy~\cite{gao20192} introduces significant redundancy due to substantial frame overlap, which is common in video data. We argue that this overlap presents an opportunity to adopt test-time augmentation (TTA), leveraging the redundant information to enhance robustness and improve prediction accuracy. We introduce Test-time Dynamic Scene Simulation (TDSS), which divides the video into $N$ sets of five consecutive frames and applies five-crop augmentation to each set across the entire video.
To summarise, our main contributions are
\begin{itemize}[topsep=0pt]
    \item An audio-visual conditional normalisation layer that adjusts feature statistics based on visual context to enhance spatial control in difference audio decoding process.
    \item A novel audio-visual contrastive learning method that enhances spatial sensitivity by mining negative samples from nearby frames and spatially shuffled visual features to simulate object position changes.
    % \item A cost-efficient approach for applying TTA to video data, improving robustness and prediction accuracy.
    \item A cost-efficient \textit{Test-time Dynamic Scene Simulation (TDSS)} strategy that exploits frame redundancy from sliding window inference by applying five-crop augmentation to consecutive frame sets for improved robustness and accuracy.
\end{itemize}
We demonstrate the effectiveness of our CCStereo model
on established benchmarks, including the FAIR-Play dataset~\cite{gao20192} with both the original 10-split~\cite{gao20192} and the more challenging 5-split protocols~\cite{xu2021visually}. 
Additionally, we extend our evaluation to two real-world datasets, MUSIC-Stereo~\cite{xu2021visually} and YT-MUSIC~\cite{morgado2018self}, demonstrating better generalisation across diverse audio-visual scenarios and superior generation quality with an efficient architecture.
% through comprehensive evaluations 
% Additionally, we extend our evaluation to the MUSIC-Stereo dataset~\cite{xu2021visually}, showcasing the model's generalisation across diverse audio-visual scenarios. Results consistently highlight that our approach achieves superior generation quality with a more efficient architecture. Code will be available.

% \begin{itemize}
%     \item \textbf{SPADE.} Utilising mean and variance in normalisation layers to control the image style is a well-study problem in computer vision. These approaches stem from the observation that content and style in data (like images or audio) can be disentangled, with mean and variance playing a key role in representing style. It is also evident that such a method can perform well in separating speaker and content information in speech synthesis. Motivated by this observation we adopted this technique for the binaural generation problem. We try to use the visual information to condition the decoding of different audio.
%     \item \textbf{Contrastive learning.} Increase model spatial sensitivity by doing contrastive learning on audio-visual cross-attention feature maps between 
%     nearby frames and randomly shuffled visual features on the spatial dimension. The random shuffling strategy may improve the volume of contrastive sets under small datasets.
%     \item \textbf{TTA.} We observe that the sliding window inference procedure contains a lot of redundancy information (i.e., a large amount of frame overlap), which is also a common issue in multi-modal learning problems. We leverage this redundant information to perform TTA, which adds zero additional cost compared with the traditional TTA.
%     \item \textit{Constrain the model with phase difference on original audio.} The phase of the difference audio is inherently linked to the phases of the left and right channels, but it does not fully represent the binaural phase dynamics.
% \end{itemize}

\begin{figure*}[ht]
    \centering
    % Dummy image using LaTeX's built-in command
    \includegraphics[width=\textwidth]{figures/mm2025-framework.drawio.pdf} % Use a placeholder image
    % \vspace{-10pt}
    \caption{
    % Illustration of our \textbf{CCStereo} method. \yuanhong{update the notation}
    Illustration of our \textbf{CCStereo} method during training. Given a pair of mono audio signals, $\mathbf{a}^{M}_{i,t}$, and a corresponding video frame, $\mathbf{v}_{i,t}$, as input, the objective is to predict the spectrogram of the difference audio, $\hat{\mathbf{a}}^{D}_{i,t}$, using a U-Net model~\cite{ronneberger2015u}. 
    \revise{
    The model comprises an image encoder network ($f_\phi$), an audio encoder network ($f_\gamma$), and an audio decoder network ($f_\psi$), which incorporates an Audio-Visual Adaptive De-normalisation (AVAD) layer to enhance feature adaptation.
    }
    % 
    The overall training objective consists of two tasks: 1) accurately reconstructing $\hat{\mathbf{a}}^{D}_{i,t}$, and 2) a contrastive learning task aimed at learning discriminative representations concerning spatial changes.
    }
    % \vspace{-10pt}
    \label{fig:framework}
    \Description[Overview of method CCStereo method]{Overview of method CCStereo method. The model comprises an encoder network, $f_\gamma$, and a decoder network, $f_\psi$, which incorporates an Audio-Visual Adaptive De-normalisation (AVAD) layer to enhance feature adaptation.}
\end{figure*}




==> tables/fairplay_music.tex <==
\begin{table*}[ht]
    \centering
    \def\arraystretch{1.1}
    \caption{
    Comparison with existing approaches on \textbf{FAIR-Play (5-splits)}~\cite{gao20192,xu2021visually} and \textbf{MUSIC-Stereo} dataset~\cite{zhao2018sound,xu2021visually}. Where \ding{72} denotes that the model uses additional data from the MUSIC21-Solo~\cite{liu2024visually} dataset, and the results in \colorbox{gray!25}{gray} indicates a reproduced implementation of the method.
    Best results are shown in \textbf{bold}, and the $2^{nd}$ best are \underline{underlined}.}
    % \vspace{-5pt}
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{!{\vrule width 1.1pt}l!{\vrule width 1.1pt}ccccc!{\vrule width 1.1pt}ccccc!{\vrule width 1.1pt}}
    \specialrule{1.1pt}{0pt}{0pt}
    % 
    % 
    \multirow{2}{*}{Methods} & \multicolumn{5}{c!{\vrule width 1.1pt}}{FAIR-Play (5-splits)~\cite{gao20192,xu2021visually}} & \multicolumn{5}{c!{\vrule width 1.1pt}}{MUSIC-Stereo~\cite{zhao2018sound,xu2021visually}}\\
    \cline{2-11}
    ~ & $\text{STFT} \downarrow$ & $\text{ENV} \downarrow$ & $\text{Mag} \downarrow$ & $ \text{Phs} \downarrow$ & $\text{SNR} \uparrow $ & $\text{STFT} \downarrow$ & $\text{ENV} \downarrow$ & $\text{Mag} \downarrow$ & $ \text{Phs} \downarrow$ & $\text{SNR} \uparrow $ \\ 
    \specialrule{1.1pt}{0pt}{0pt}
    Mono-Mono~\cite{xu2021visually} & 1.024 & 0.145 & 2.049 & 1.571 & 4.968 & 1.014 & 0.144 & 2.027 & 1.568 & 7.858 \\ 
    Mono2Binaural~\cite{gao20192, xu2021visually} & 0.917 & \underline{0.137} & 1.835 & 1.504 & 5.203 & 0.942 & 0.138 & 1.885 & 1.550 & 8.255 \\ 
    % PseudoBinaural (w/o sep.)~\cite{xu2021visually} & 0.951 & 0.140 & 1.914 & 1.539 & 5.037 & 0.953 & 0.139 & 1.902 & 1.564 & 8.129 \\ 
    PseudoBinaural~\cite{xu2021visually} & 0.944 & 0.139 & 1.901 & 1.522 & 5.124 & 0.943 & 0.139 & 1.886 & 1.562 & 8.198 \\ 
    Sep-Stereo~\cite{zhou2020sep, xu2021visually} \ding{72} & \underline{0.906} & \textbf{0.136} & \underline{1.811} & 1.495 & 5.221 & 0.929 & 0.135 & 1.803 & 1.544 & 8.306 \\ 
    CMC~\cite{liu2024visually} & \cellcolor{gray!25} 0.912 & \cellcolor{gray!25} 0.141 & \cellcolor{gray!25} 1.824 & \cellcolor{gray!25} 1.502 & \cellcolor{gray!25} 6.238 & 0.759 & 0.113 & 1.518 & \textbf{1.502} & - \\
    BeyondM2B~\cite{parida2022beyond} & 0.909 & 0.139 & 1.819 & \underline{1.479} & \underline{6.397} & \underline{0.670} & \underline{0.108} & \underline{1.340} & \underline{1.538} & \underline{10.754} \\ 
    \hline
    \rowcolor{LightCyan}\textbf{CCStereo} & \textbf{0.883} & \underline{0.137} & \textbf{1.766} & \textbf{1.454} & \textbf{6.475} & \textbf{0.624} & \textbf{0.097} & \textbf{1.248} & 1.578 & \textbf{12.985} \\
    % Ours - R50 & 0.887 & 0.137 & 1.773 & 1.453 & 6.434 & 0.605 & 0.097 & 1.209 & 1.574 & 12.748 \\ 
    \specialrule{1.1pt}{0pt}{0pt}
    % 
    % 
    \end{tabular}
    % }
    \label{tab:fairplay_music}
    % \vspace{-5pt}
 \end{table*}
